POLAR-Express: Efficient and Precise Formal Reachability Analysis of Neural-Network Controlled Systems

Neural networks (NNs) playing the role of controllers have demonstrated impressive empirical performances on challenging control problems. However, the potential adoption of NN controllers in real-life applications also gives rise to a growing concern over the safety of these neural-network controlled systems (NNCSs), especially when used in safety-critical applications. In this work, we present POLAR-Express, an efficient and precise formal reachability analysis tool for verifying the safety of NNCSs. POLAR-Express uses Taylor model arithmetic to propagate Taylor models (TMs) across a neural network layer-by-layer to compute an overapproximation of the neural-network function. It can be applied to analyze any feed-forward neural network with continuous activation functions. We also present a novel approach to propagate TMs more efficiently and precisely across ReLU activation functions. In addition, POLAR-Express provides parallel computation support for the layer-by-layer propagation of TMs, thus significantly improving the efficiency and scalability over its earlier prototype POLAR. Across the comparison with six other state-of-the-art tools on a diverse set of benchmarks, POLAR-Express achieves the best verification efficiency and tightness in the reachable set analysis.

==> sections/experiment.tex <==
\section{Comparison and Experimental Results}\label{sec:experiment}

\subsection{Progress}
\begin{table}[ht]
\centering
\caption{Experiment Progress Record}
\begin{tabular}{|l|c|c|c|c|}
\hline
Example    & Polar & Verisig & CROWN+flow* &  NNV \\ \hline
Benchmark1 & Y     &     Y    &      Y       &  Y \\ \hline
Benchmark2 & Y     &      Y   &      Y       & Y \\ \hline
Benchmark3 & Y     &      Y   &     Y        & Y \\ \hline
Benchmark4 & Y     &      Y   &     Y        & Y \\ \hline
Benchmark5 & Y     &     Y    &     Y        &  Y \\ \hline
Benchmark6 & Y     &    Y     &     Y        &  Y \\ \hline
Attitude Control        & Y     & Y       &      Y       & Y \\ \hline
ACC        & Y     & Y       &     Y        & Y \\ \hline
Quadrotor  & Y     & Y       &             & --  \\ \hline
MC         & Y     &    Y     &       Y      & Y  \\ \hline
\end{tabular}
\end{table}



==> sections/methods.tex <==
\section{Overview of Methods}\label{sec:methods}

\chen{Move the two lemmas from the arXiv paper to here.}


\iffalse
We describe the existing techniques for overapproximating the reachable sets of NNCSs from the methodology point of view.
Most of the existing reachability analysis methods use a set-propagation scheme to compute overapproximate reachable set segments which are often called \emph{flowpipes} over a finite number $K$ of control steps. The main framework is presented by Algorithm~\ref{algo:flowpipe_nncs}. We briefly explain the steps there.


Starting with a given initial set $X_0$, the main algorithm repeatedly performs the following two main steps to compute the flowpipes in the $(i+1)$-st control step for $i = 0,1,\dots, K-1$:

\noindent (a) \emph{Computing the control input range $\mathcal{U}_i$.} This task is to compute the output range of $h \circ \kappa \circ g \circ \pi(\mathcal{X}_i)$ and is performed by the statements in Line 3 to 6. The key step is Line 5 which computes a set that is guaranteed to contain the NN output range. In the paper, our experiments will investigate the effectiveness of the interval, ImageStar, and Taylor model representations for the set $\mathcal{V}_i$ in the NNCS reachability analysis framework.


\noindent (b) \emph{Flowpipe computation for the continuous dynamics.} It computes flowpipes each of which is guaranteed to contain the actual reachable states in a sub time interval in the current control step. This task can be done using the existing methods or tools such as CORA and Flow*. The set $\mathcal{X}_i$ for the next step can be obtained by evaluating the last flowpipe at the end of its time interval. Since the control inputs modify the continuous dynamics instead of directly change the the system states, only the flowpipes are considered in the final overapproximation set.






\begin{algorithm} [t]
 \caption{Reachable set computation for NNCSs based on set-propagation.}\label{algo:flowpipe_nncs}
 \begin{algorithmic}[1]
  \REQUIRE Definition of the system modules, number of control steps $K$.
  \ENSURE Overapproximation of the reachable set over the time interval of $[0, K\delta_c]$ wherein $\delta_c$ is the control stepsize.
  \STATE $\mathcal{R} \leftarrow \emptyset$; \COMMENT{the resulting overapproximation set}
  \FOR{$i=0$ to $K-1$}
   \STATE Computing an overapproximation $\mathcal{Y}_i$ for the range $\pi(\mathcal{X}_i)$;
   \STATE Computing an overapproximation $\mathcal{Z}_i$ for the range $g(\mathcal{Y}_i)$;
   \STATE \textbf{Computing an overapproximation $\mathcal{V}_i$ for the range $\kappa(\mathcal{Z}_i)$;}
   \STATE Computing an overapproximation $\mathcal{U}_i$ for the range $h(\mathcal{V}_i)$;
   \STATE Computing a set $\mathcal{F}$ of flowpipes for the continuous dynamics $\dot{\vx} = f(\vx,\vu)$ with $\vu\in \mathcal{U}_i$ from the initial set $\vx(0) \in \mathcal{X}_i$ over the time interval of $[i\delta_c,(i+1)\delta_c]$;
   \STATE $\mathcal{R} \leftarrow \mathcal{R} \cup \mathcal{F}$;
   \STATE Evaluating an overapproximation for the reachable set at the time $t = (i+1)\delta_c$ based on $\mathcal{F}$ and assigning it to $\mathcal{X}_{i+1}$;
  \ENDFOR
  \RETURN $\mathcal{R}$.
 \end{algorithmic}
\end{algorithm}
\fi

%The set-propagation methods can be mainly classified to the following two groups based on their overapproixmation purposes.

%\noindent\textbf{(I) Pure range overapproximations for reachable sets.}
%The techniques in this group aim at directly overapproximating the range of the reachable set using geometric or algebraic representations such as intervals, zonotopes or other sets represented by constraints. Such an approach can often be developed by designing the overapproixmation methods for the plant and controller individually, and then use a higher-level algorithm to make the two methods work cooperatively for the closed-loop system. Many existing tools for computing the reachable set overapproximations under the continuous dynamics defined by linear or nonlinear ODEs can be used to handle the plant, such as VNODE-LP\cite{Nedialkov/2011/vnode-lp}, SpaceEx~\cite{Frehse+/2011/SpaceEx}, CORA~\cite{Althoff/2015/CORA}, and Flow*~\cite{Chen+/2013/flowstar}. On the other hand, the task of computing the output range of a neural network can be handled by the output range analysis techniques most of which are developed in the recent years~\cite{duttoutputa2018, tjeng2019evaluating, cheng2017maximum, Lomuscio+Maganti/2017/Approach,huang2017safety,katz2017reluplex,ruan2018reachability,gehr2018ai2, singh2018fast,wang2018formal,tran2020nnv,zhang2018efficient,wang2021beta}.
%The main advantage of the techniques in this group is twofold. Firstly, there is no need to develop a new technique from scratch, and the correctness of the composed approach can be proved easily based on the correctness of the existing methods for the subtasks. Secondly, the performance of the approach is often good on simple case studies since it can use well engineered tools as primitives. However, since those methods mainly focuses on the pure range overapproximation work, and do not or just lightly track the dependencies among the state variables under the system dynamics, it may cause heavy accumulation of overapproximation error when the plant dynamics is nonlinear or the initial set is large, make the resulting bounds less useful in proving properties of interest.


%on the other hand,  the relationship between the control inputs and the plant states are not explicitly represented in this approach. This  may lead to a overestimation when the plant dynamics is nonlinear or the initial set is large, making the resulting bounds less useful in proving properties of interest.



%\begin{figure}[t]
%    \centering
%    \includegraphics[width = 9cm]{figs/TM_flowpipe.png}
%    \caption{Taylor model overapproximation of a flowmap function.}
%    \label{fig:tm_flowpipe}
%\end{figure}


%\noindent\textbf{(II) Functional overapproximations for system evolution.}
%The reachable set overapproximation methods in this category focus on a more challenging task than only overapproximating the reachable set ranges. They seek to compute an overapproximate function for the flowmap $\Phi$ of an NNCS. As we pointed out in the previous section, $\Phi$ is a function only in the variables representing the initial state and the time, and it often does not have a closed-form expression. However, it can be overapproximated by a Taylor model (TM) over a bounded time interval. Figure~\ref{fig:tm_flowpipe} gives an illustration in which the TM $p(\vx_0,t_0+\tau) + [a,b]$ is guaranteed to contain the range of the function $\Phi(\vx_0,t_0 + \tau)$ for any initial state $\vx_0$ and $t\in [0,\delta]$. In practice, we usually require $\vx_0$ to be in a bounded set. Such a TM provides a functional overapproximation rather than a pure range overapproximation which allows to track the dependency from a reachable state to the initial state approximately.
%Functional overapproximations often can handle more challenging reachability analysis tasks, in which larger initial sets, nonlinear dynamics, or longer time horizons are specified.
%Recent work has applied interval, polynomial and TM arithmetic to obtain overapproximations for NNCS evolutions~\cite{Dutta_Others__2019__Reachability,huang2019reachnn,IvanovCWAPL21,huang2021polar}. Those techniques are often able to compute more accurate flowpipes than the methods in the other group. On the other hand, the functional overapproximation methods are often computationally expensive due to the computation of nonlinear multivariate polynomials for tracking the dependencies.

\iffalse
\begin{table}[t]
    \centering
    \caption{Summary of the tools evaluated in this paper.}
    \label{tab:tool_summary}
    \begin{adjustbox}{width=.95\columnwidth}
        \begin{tabular}{@{}c|c|c|c|c@{}}
            \toprule
            Tool & Category & \stackanchor{Plant}{Dynamics} & \stackanchor{Activation}{Function} & \stackanchor{Set}{Representation} \\
            \midrule
            \midrule
            \stackanchor{$\alpha,\beta$-CROWN}{+ Flow*} & (I) & nonlinear & continuous & \stackanchor{Interval and}{Taylor model} \\
            \midrule
            NNV & (I) & \stackanchor{discrete linear,}{continuous (CORA)} & \stackanchor{ReLU, tanh,}{sigmoid} & ImageStar \\
            \midrule
            POLAR & (II) & nonlinear & continuous & Taylor model \\
            \midrule
            Verisig 2.0 & (II) & nonlinear & differentiable & Taylor model \\
            \midrule
            \zhou{Juliareach} & (II) & nonlinear & differentiable & Zonotope + Taylor model \\
            \midrule
            \zhou{CORA} & (II) & nonlinear & differentiable & Polynomial zonotope \\
            \midrule
            RINO & (II) & nonlinear & differentiable & interval + interval Taylor series \\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table}
\fi


\noindent\textbf{Tool selection.} Table~\ref{tab:tool_summary} presents all of the tools which will be involved in our experimental evaluation. In order to consider more types of activation functions, the tools which can only handle particular types of activation functions, such as Sherlock, are not selected. Besides their categories, we also consider the following key functionalities and features. Plant dynamics denotes the type of continuous dynamics which can be handled by the tool. Since all of the tools except NNV use Flow* to handle the continuous dynamics, they can support nonlinear ODEs. NNV natively works on linear discrete plant dynamics, however may deal with nonlinear ODEs with the help of CORA. Similar to NNV, $\alpha,\beta$-CROWN is also a tool mainly focusing on the output range analysis of NNs, we build a ``new'' tool which simply combines the use of $\alpha,\beta$-CROWN and Flow* to handle NNCSs, such that the output range obtained from the former tool is represented by an interval. Although $\alpha,\beta$-CROWN supports other representations than intervals for NN output ranges, only intervals can be directly used by existing reachability tools for ODEs. 



%  \begin{table*}
% \caption[Caption for LOF]{A summary of NNCS verification methods in this paper.}
% \centering
% \begin{adjustbox}{width=0.8\columnwidth}
% \begin{threeparttable}
% \begin{tabular}{@{}ccc@{}}
% \toprule
% Methods & Plant Dynamics & Activation Function \\ \midrule
% POLAR & Discrete, Continuous, Hybrid & ReLU, sigmoid, tanh \\ \midrule
% Verisig 2.0 & Discrete, Continuous, Hybrid & sigmoid, tanh \\ \midrule
% alpha-beta CROWN + Flow* & Discrete, Continuous, Hybrid & ReLU, sigmoid, tanh \\ \midrule
% NNV & Discrete, Continuous & ReLU, sigmoid, tanh \\ \bottomrule
% \end{tabular}
% \end{threeparttable}
% \end{adjustbox}
% \label{tab:method_features}
% \end{table*}
 

==> sections/weichao.tex <==
\section{A Collection of Dynamical Models}

\subsection{Bicycle model}
 
A bicycle model and one of its extension can be found in~\cite{7353998}. The extension replaces the wheels of the model with omnidirectional wheels that move in two orthogonal directions independently to simulate beveled-tip needle motion in soft tissue.

\subsection{Electro-hydraulic system}

An electro-hydraulic system is formalized in~\cite{6224628} where the system is used to produce torque to actuate a robot. There are $4$ state variables and $3$ inputs. 
\begin{eqnarray}
\dot{F}&=&f(\textbf{P}, x_p) + g(\textbf{P}, \dot{x}_p) u\nonumber\\
g(\textbf{P}, x_p)&=&K_v A_p \beta [\frac{\sqrt{P_S- P_A}}{V_A(x_p)}+\frac{\alpha\sqrt{P_B - P_T}}{V_B(x_p)}]\nonumber\\
f(\textbf{P}, \dot{x}_p)&=&-A^2_p \beta [\frac{1}{V_A(x_p)} + \frac{\alpha^2}{V_B(x_p)}]\dot{x}_p\nonumber
\end{eqnarray}

\subsection{Quadrupedal robot}

A quadrupedal robot is studied in~\cite{8793669}. The dynamical model has $4$ state variables ${x}:=[{p}, {\dot{p}}, {R}, \omega^B]$ respectively representing the position, velocity, rotation matrix and angular velocity. Additionally, $M$ is the mass of the rigid body; $a_g$ is the gravitional acceleration; $I^B$ is the fixed moment of inertia tensor in the body.
\begin{eqnarray}
\dot{x}=f({\dot{x}}, {\dot{u}})=\begin{bmatrix}{\dot{P}} \\ \dot{P} \\ {\dot{R}} \\ {\dot{\omega}^B}\end{bmatrix}=\begin{bmatrix}{\dot{P}} \\ \frac{f}{M}-a_g \\ R\cdot \omega^B \\ {I^B}^{-1}(R^T \tau - \hat{\omega}^B I \omega)\end{bmatrix}\nonumber
\end{eqnarray}

\subsection{Quadrotor}

A quadrotor dynamics is introduced in \cite{9636485} as below where $r$ is position, $v$ is velocity, $R$ is a rotation matrix, $\omega$ is the angular velocity expressed in the body frame, $T$ is the cumulative thrust generated by the four propellers; the input $\mu_{\delta T}$ controls the derivative of the thrust; $\mu_\tau$ is the torque applied to the quadrotor in the body frame; $J$ is the quadrotor's inertia matrix; $e_3=[0, 0, 1]^T$. The state of the system is $(r, v, R, \omega, T)$ and the control is its time derivative. The control goal is to stay in a the safe set which is a union of polytopes.
\begin{eqnarray}
\dot{r}&=& v\nonumber\\
\dot{v} &=& \frac{1}{m}(TRe_3-mge_3)\nonumber\\
\dot{R} &=& R[\omega\times]\nonumber\\
\dot{T} &=& \mu_{\delta T}\nonumber\\
J\dot{\omega} &=& \mu_T - [\omega\times] J\omega\nonumber
\end{eqnarray}

==> sections/zhilu.tex <==
\subsection{Another quadrotor control system}
This quadrotor control system is from~\cite{verisig2}. The goal is to let the quadrotor follows a piecewise-linear trajectory. The system has 6-dim states $x, y, z, \Dot{x}, \Dot{y}, \Dot{z}$ with 3-dim control input $\theta, \phi, \tau$ (controls the angular acceleration for pitch, roll and thrust).
\begin{gather*}
    \Dot{x} = g \tan(\theta)\\
    \Dot{y} = -g \tan(\phi)\\
    \Dot{z} = \tau - g
\end{gather*}
The NN controller in~\cite{verisig2} is learned from an MPC controller.

\subsection{ACC}
\subsubsection{ACC with disturbance}
This ACC model is from~\cite{wang_2021_emsoft}. The ego vehicle ODE is $\Dot{y}_e = v_e$, $\Dot{v}_e = a_e - k v_e$, where $k$ is the resistance coefficient. The reference vehicle ODE is $\Dot(y)_r = v_r$. Vehicle distance is $\Delta y = y_r - y_e$. The ACC controller controls the distance and the ego car velocity to the equilibrium $\Delta \Bar{y} = 80$, $\Bar{v} - 30$ and maintain the safe range: $|\Delta y - \Delta \Bar{y}|\leq 40$, $|v_e - \Bar{v}|\leq 10$. $v_r$ is assumed to be bounded $|v_r - \Bar{v}|\leq 8$. System dynamic is:
\begin{equation*}
    \Dot{x} = 
    \begin{bmatrix}
    0 & -1\\
    0 & -k
    \end{bmatrix} x + 
    \begin{bmatrix}
    0\\
    1
    \end{bmatrix} u + 
    \begin{bmatrix}
    1\\
    0
    \end{bmatrix} w
\end{equation*}
where system state $x = [\Delta y - \Delta \Bar{y}, v_e - \Bar{v}]^\top$, control input $u = a_e - k\Bar{v}$, and disturbance $w = v_r - \Bar{v}$.

RL-based controller can be found in~\cite{Yixuan_2020_ICCAD}.

\subsubsection{ACC with known reference dynamics}
This ACC model is used in Verisig~\cite{verisig2}.
\begin{gather*}
    \Dot{y}_e = v_e,\ \Dot{v}_e = a_e, \\
    \Dot{a}_e = 2u - 2a_e - 0.001v_e
\end{gather*}
\begin{gather*}
    \Dot{y}_r = v_r,\ \Dot{v}_r = a_r, \\
    \Dot{a}_r = -4 - 2a_r - 0.001v_r
\end{gather*}

Initial set: $y_e(0)\in[10,11]$, $v_e(0)\in[30, 30.05]$, $a_e(0)=0$, $y_r(0)\in[90,91]$, $v_r(0)\in[32, 32.05]$, $a_r(0)=0$.

Goal region: $y_e\in[29.88, 30.02]$, $y_r\in[22.81,22.87]$. 

Unsafe region (interpreted from code): $y_r - y_e - 10 - 1.4 v_e \leq 0$.

NN controller: a tanh NN on Github: 5-dim input, 1-dim output. The input includes (not sure) $f_1=y_r - y_e - 10 - 1.4 v_e$, $f_2=1.4$ (?), $f_3 = v_e$, $f_4 = y_r - y_e$, $f_5 = v_r - v_e$.

\subsection{Unprotected left turn}
This model is from a just-accepted paper from Xiangguo Liu. The system is a 5-dimention, time-variant system:
\begin{gather*}
    \Dot{y_1}=v_1\\
    \Dot{v_1}=u\\
    \Dot{\tau}_{\min}=f_1(t)\\
    \Dot{\tau}_{\max}=f_2(t)\\
    \Dot{t} = 1
\end{gather*}
where $y_1$, $v_1$ is the position and velocity of the left-turn vehicle. $[\tau_{\min},\tau_{\max}]$ is the prediction of the time window when the go-straight vehicle crosses the intersection. The predicted time window is assumed to be tighter as two vehicles get closer, i.e., $f_1(t)\geq 0$, $f_2(t)\leq 0$. 

Initial set: $y_1\in[-60.4, -60.3]$, $v_1\in[10.5, 10.51]$, $\tau_{\min} = 14$, $\tau_{\max} = 16$, $t=6$.

Unsafe region: $\{t\in [\tau_{\min},\tau_{\max}]\} \bigcap \{y_1\in[4.5, 14]\}$.

NN controller: Yes.

\subsection{2-link robot arm control}

This model is from~\cite{Guechi_2018_robotarm}, which is a non-linear system with 4-dim states and 2-dim control input (controls the torque of each arm).

Initial set, goal, unsafe set: TBD

NN controller: TBD

\subsection{Van der Pol's Oscillator}

The 2-dim model can be found in~\cite{wei2019general} as:
\begin{equation*}
    \Ddot{x}+(x^2 - 1)\Dot{x} + x = u
\end{equation*}

RL-based controller can be found in~\cite{Yixuan_2020_ICCAD}.

\subsection{Cartpole system}
4-dim discretized dynamics, and the coresponding RL-based controller can be found in~\cite{yixuan2021cocktail}.

\subsection{Mountain Car}
2-dim discrete system in~\cite{verisig2} with RL controller.
\begin{gather*}
    x[t+1] = x[t] + v[t]\\
    v[t+1] = v[t] + 0.0015u[t] - 0.0025 \cos(3x[t])
\end{gather*}
And the control input is restricted in $[-1, 1]$.

\subsection{More examples}

The ODEs of more examples with 2-5 state variables can be find in~\cite{sassi2017linear}.

==> weichaozhou/benchmarks/acc.tex <==
The Adaptive Cruise Control (ACC) benchmark is a system composed of two vehicles maintaining a safe distance between each other. One vehicle is a lead vehicle and the other one is an ego vehicle. The system dynamics is:
\begin{equation*}
% \label{4.8.1}
\begin{aligned}
\dot{x}_{lead} = v_{lead}, &\quad \dot{v}_{lead}=\gamma_{lead}, &\quad \dot{\gamma}_{lead} =-2\gamma_{lead} + 2 a_{lead} - u v^2_{lead},\\
\dot{x}_{ego} = v_{ego}, &\quad \dot{v}_{ego}=\gamma_{ego}, &\quad \dot{\gamma}_{ego}=-2\gamma_{ego}+ 2 a_{ego} - u v^2_{ego},
\end{aligned}
\end{equation*}
where $x$ is position. $v$ is velocity. $\gamma$ is acceleration. And $u=0.0001$ is a friction coefficient.

Given a constant $a_{lead}\equiv -2$, an NN controller computes an optimal control thrust $a_{ego}$ such that the ego vehicle travels at a set speed $v_{set}= 30$, and the relative distance $D_{rel}:=x_{lead}-x_{ego}$ is no less than a safe distance $D_{safe}:=D_{default} + T_{gap}\times v_{ego}$ where $D_{default}=10$ and $T_{gap}=1.4$. The input to the neural network controller is $v_{set}, T_{gap}, v_{ego}, D_{rel}, v_{rel}$. The initial set is $x_{lead}\in[90, 91], v_{lead}\in[32, 32.05], \gamma_{lead}=\gamma_{ego} = 0, v_{ego}\in[30, 30.05], x_{ego}\in[10, 11]$.
The target is $v_{lead} \in [22.81, 22.87]$ and $v_{ego} \in [29.88, 30.02]$.
The total control steps $N$ is 50 and the control period is 0.1 seconds. The derived reachable sets and simulation traces are shown in Figure~\ref{fig:acc}.

\begin{figure}[pbh!]
    \centering
    \includegraphics[width=0.5\columnwidth]{./figs/benchmarks/ACC.pdf}
    \caption{Results of ACC. POLAR for 50 steps (blue sets), Verisig 2.0 for 50 steps (grey sets), $\alpha,\beta$-CROWN\,+\,Flow* for 50 steps (green sets), NNV for 50 steps (yellow sets), and simulation traces for 50 steps (red curves).}
    \label{fig:acc}
\end{figure}

==> weichaozhou/benchmarks/docking.tex <==
% \chen{The state variables are changed to 5 in Example 1.}

The 2D spacecraft docking benchmark is first introduced in Example~\ref{exam:docking} of Section~\ref{sec:problem}. We consider an NN controller trained in~\cite{ravaioli2022safe} to perform control every second. 
The initial set is defined by $x, y\in[24, 26]$, $v_x=v_y= -0.1378$, and $v_{safe}\in [0.2697, 0.2755]$ which is directly computed based on the ranges of $x, y$.  
The total control steps $N$ is $100$.
In this benchmark we focus on verifying the safety property. 
That is, the NN controller should maintain $\sqrt{v_x^2 + v_y^2}\leq v_{safe}$ all the time. 
As in Figure~\ref{fig:docking}, where the x and y-axis are respectively $v$ and $v_{safe}$, the blue borderline partitions the safe and unsafe regions. 




\begin{figure}[h!]
    \centering
	\includegraphics[width=0.5\textwidth]{figs/benchmarks/docking_new.pdf}%
    \caption{Results of 2D Spacecraft Docking. POLAR for 100 steps (blue sets),
    % \li{showing 100 steps is probably good enough; although if 120 is when Flow* exits in POLAR, then we should keep it and say we run until this termination condition is met}, 
    Verisig 2.0 for 7 steps (grey sets)
    , $\alpha,\beta$-CROWN\,+\,Flow* for 14 steps (green sets), and NNV for 13 steps (yellow sets), and simulation traces for 100 steps (red curves).}
    \label{fig:docking}
\end{figure}

